Labeled Interactive Topic Models

Topic models are valuable for understanding extensive document collections, but they don't always identify the most relevant topics. Classical probabilistic and anchor-based topic models offer interactive versions that allow users to guide the models towards more pertinent topics. However, such interactive features have been lacking in neural topic models. To correct this lacuna, we introduce a user-friendly interaction for neural topic models. This interaction permits users to assign a word label to a topic, leading to an update in the topic model where the words in the topic become closely aligned with the given label. Our approach encompasses two distinct kinds of neural topic models. The first includes models where topic embeddings are trainable and evolve during the training process. The second kind involves models where topic embeddings are integrated post-training, offering a different approach to topic refinement. To facilitate user interaction with these neural topic models, we have developed an interactive interface. This interface enables users to engage with and re-label topics as desired. We evaluate our method through a human study, where users can relabel topics to find relevant documents. Using our method, user labeling improves document rank scores, helping to find more relevant documents to a given query when compared to no user labeling.

==> sections/50-study.tex <==

To validate the efficacy of \abr{i-ntm}, we recruited participants to test our
model in finding more relevant documents for different scenarios and
information needs. Information retrieval tasks are an intuitive way to measure
the success of our method, since they involve finding relevant information
specific to a query. Comparing the scores from these scenarios, before and
after labeling, is used to verify that user labeling brings forth more
relevant documents. We find users do relabel at least one topic on average and
the labeling does improve ranking scores on a common information retrieval
algorithm.

\subsection{Setup}
To conduct this study, we recruited 20 participants through the online platform Prolific, whom were given one hour to complete the task. Our study is set up as follows:
\begin{enumerate}
    \item Our model \abr{i-ntm} is used to generate topics on a dataset related to disaster relief situations\footnote{we chose the \abr{better} disaster relief dataset mentioned throughout the paper since it has documents sorted into different scenarios with questions already given. }
    \item Participants are shown an information need with topics generated by our model. After consideration, they have the opportunity to label topics in a way they deem best
    \item After labeling topics, they are asked to select a few documents that they believe best answer the information need \kscomment{I think a good point was brought up here, a "few documents" is vague, should keep it consistent frome each user so tell them how many to label otherwise one user could label 1 and one users could label 10}
\end{enumerate}

For each user we collected the topic information and document distribution before and after the human interaction. Then following the algorithm commonly known as BM25 \citep{Robertson1994OkapiAT}, an information retrieval ranking function. We compare the estimated relevancy of topics before and after the human interaction. BM25 works by using a bag-of-words retrieval function that ranks a set of documents based on query terms present in the document. 

\subsection{Results}

\jbgcomment{I think psychologically to some of the reviewers, the lack of ink on the results made them seem insignificant.  Perhaps we could:

  - Talk about the kinds of changes users did (i.e., help them understand what kinds of labels were added)
  
  - Talk about how the embeddings change with updates (internal to the model)

  - Talk about how the topics changes with updates (visible to the user)

  - Talk about latencies

  - Talk about which updates worked and which didn't, and you can contrast this with the original ITM paper.  E.g., are there effects from embeddings, polysemy, etc.

}

In Figure~\ref{fig:study} we see the average BM25 document ranking scores for each question averaged over the 20 users. We show the scores for the topics that were changed, before and after the users made the change. This shows that on average, changing the topic led to more representative documents being shown (when looking at up to the first 5 documents for each topic). \kscomment{reviewer asked why no bar for q2, it is answered here, but maybe can make it more clear} In the case of \textit{Q2} and \textit{Q9}, no \textit{Before update} bar is present because some topics initially had no documents clustered under that topic. We believe that due to the limited size of the dataset, a few topics covered a majority of the documents, causing some topics to have no documents clustered to it. 
%
Figure \ref{fig:study_plot} shows how over the course of the study, as the user labels topics for more scenarios, the overall document ranking score increases. This is demonstrating how for a given corpus, by labeling topics for different questions, one can incremently increase overall document relevancy. This figure also shows the average number of new documents associated with the new topics that the user labels. A high number of new associated documents, does not necessarily correlate with a larger increase in document ranking score, as some low ranked documents could pull down the rest. 



\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/study.png}
    \caption{Average BM25 document ranking scores for each of the 10 questions averaged, over the 20 users. }
    \label{fig:study}
\end{figure}



